Planning for Muscular and Peripersonal-Space Comfort during Human-Robot Forceful Collaboration

This paper presents a planning algorithm designed to improve cooperative robot behavior concerning human comfort during forceful human-robot physical interaction. Particularly, we are interested in planning for object grasping and positioning ensuring not only stability against the exerted human force but also empowering the robot with capabilities to address and improve human experience and comfort. Herein, comfort is addressed as both the muscular activation level required to exert the cooperative task, and the human spatial perception during the interaction, namely, the peripersonal space. By maximizing both comfort criteria, the robotic system can plan for the task (ensuring grasp stability) and for the human (improving human comfort). We believe this to be a key element to achieve intuitive and fluid human-robot interaction in real applications. Real HRI drilling and cutting experiments illustrated the efficiency of the proposed planner in improving overall comfort and HRI experience without compromising grasp stability.

==> New folder/Comfort/Comfort.tex <==
\section{Muscular Comfort}
\label{sec:Muscular} 

This section introduces the metric used to quantify human muscular comfort, given a candidate configuration of the human-robot system and the forceful operation $\left(\textbf{\textit{q}}_{\text{h}}, \, _{\text{h}}{\textbf{\textit{T}}},  \, ^{\text{o}}{\textbf{\textit{f}}}, \, _{\text{t}}^{\text{o}}{\textbf{\textit{T}}}, \, _{\text{o}}{\textbf{\textit{T}}} \right)$.
This is a crucial element of the proposed system since the planner needs a
consistent quantitative assessment of human comfort to be optimized. 

To do this we model the human arm as a serial-link kinematic chain with seven
degrees of freedom (DOFs) \textemdash two spherical and one revolute joint
respectively at the shoulder, wrist and elbow \footnote{An important limitation
of this current formulation is that it only considers the human arm in the
comfort metric, and ignores the rest of the body. It is our intention to extend
the formulation and our planner to the whole body in the future.}.  The
configuration of this seven-DOF human arm is represented with the vector
$\myvec q _\human $. We use $\mymatrix{J}_\human ( \myvec q _\human )$ to
represent the geometric Jacobian of the human configuration (which we simplify
to $\mymatrix{J}_\human$ dropping the argument in this section). Furthermore,
in this section, we use $\myvec{f}$ to refer to the force the human is applying
in the world frame. Given the object pose $_\obj\mymatrix{T}$, the tool pose
$_{\text{t}}^{\text{o}}{\textbf{\textit{T}}}$, and the force in the object
frame $^\obj\myvec{f}$, $\myvec{f}$ can be found by a norm-preserving
transformation.

Assuming quasi-static movements, the effects of higher order dynamics can be
neglected and the human joint torques depend solely on the exerted force
$\myvec{f}$ and the gravity effects.  We assume the gravitational forces
results from the contribution of the upper arm and forearm weights and centre
of mass, and the tool mass and pose.  Naturally, the gravitational forces are
well-defined in the inertial/world frame and do not depend on the arm
configuration. However their gravitational torque---respectively, over the
shoulder, shoulder and elbow system and for the full arm---depends on the joint
configuration.  We use $\rho_\human(\myvec q_\human)$ to refer to these
generalized gravitational forces for a given human arm configuration, and again
we drop the argument $\myvec q_\human$ in the rest of the section for clarity.

Then, for a given forceful operation and human configuration, the required torques at
the human joints can be computed using:
\begin{equation}
\myvec{\tau}_\human  =  \mymatrix J^{T}_\human ( \myvec \forcef + \myvec \rho_\human)
\label{eq:Torque Human}
\end{equation}
where $\myvec{\tau}_\human$ is the vector of torques at the human joints.

If a human arm worked exactly like a robotic manipulator, we could compare the
torque values in $\myvec{\tau}_\human$ with the torque limits of the human
joints
%, $\myvec{\tau}_\human^{\text{limits}}$, 
and we could devise a comfort metric based on how close the torque
values are to the limits; i.e. the further from the limits, the more
comfortable it would be.

However, a better modeling of how the human muscles work is presented in Tanaka
et al. \cite{2015_Tanaka_Nishikawa_Yamada_Tsuji__TransHaptics}, which we use to
build our comfort metric. There are two key differences in this model, compared
to a robotic manipulator model. When approximating human's muscular structure with a kinematic structure like ours:
\begin{itemize}
    \item The torque limits must depend on the configuration, i.e. the torque limits do not stay constant at different configurations as they do for a robot manipulator;
    \item The torque limits must depend on the direction of motion, e.g. the limits of the elbow must be modeled differently if it is flexing versus if it is extending.
\end{itemize}
This suggests that, for the human arm, we model the torque limits as a function
of the configuration and the differential change in the configuration: $\Pi (\myvec q_\human, \dot{\myvec q}_\human )$, which we represent 
as a diagonal matrix with human maximum torque elements, that is,
$\text{diag} \{\tau_{1}^{max}(\myvec q_\human, \dot{\myvec q}_\human ),\dots,\tau_{7}^{max}(\myvec q_\human, \dot{\myvec q}_\human ) \}$. 
The matrix $\mymatrix \Pi$
represents the nonlinear relationship between human torque limits and joints;
and each maximum torque element, $\tau_{i}^{max}$, is a nonlinear
function of the joint values and their directions. %which is task-dependent. 
% That is to say the maximum torque for each joint depends not only on its
% position but also on its derivative (e.g., raising and lowering the
% upper arm use different muscles). 
% 
Experimental data to compute the values for $ \mymatrix \Pi (\myvec q_\human,
\dot{\myvec q}_\human ) $ for different human arm configurations can be found
in the excel work of Tanaka et al.
\cite{2015_Tanaka_Nishikawa_Yamada_Tsuji__TransHaptics} and the values therein
are used throughout this work. 

This formulation requires us to know $\dot{\myvec q}_\human$ to extract the
direction each human joint will be moving during the forceful operation. We
compute $\dot{\myvec q}_\human$ by assuming that the human follows a
Jacobian-transpose controller: ${\myvec q}_\human=\mymatrix J_\human^T(\myvec
q_\human) \dot{\myvec x}_\human$, where $\dot{\myvec x}_\human$ is the
human hand motion during the application of the forceful operation. In this
work, we assume the hand moves in the same direction with the operational
force.

Equipped with  $\mymatrix \Pi (\myvec q_\human, \dot{\myvec q}_\human ) $, 
instead of Eq.~\ref{eq:Torque Human}, we can compute the 
human joint torque activation levels $\myvec{\alpha}_{\human}=[\alpha_{1},\dots,\alpha_{7}]^{T}$:
\begin{equation}
    \myvec{\alpha}_{\human}  =  \mymatrix \Pi^{-1} \mymatrix J^{T}_\human ( \myvec \forcef + \myvec \rho_\human)
\label{eq:Activation Level Human}
\end{equation}
where $\alpha_{i}\in[0,1]$ represents the activation ratio of the
$i$-th joint's torque $\tau_{i}$ to its maximum torque $\tau_{i}^{max}$---under maximum voluntary contraction and taking the 
muscle tension is nearly proportional to the muscle activation level. 

In this work, we use the norm of the activation level vector to compute the muscular human comfort. Specifically, we use
\begin{equation}
    \text{Muscular} ( \myvec q _\human, { _{\obj} \mymatrix{T} },  {^\obj\myvec{f}} , { ^\obj _{\tool} \mymatrix{T} } ,  { _{\obj} \mymatrix{T} } ) = 1 / ||\myvec{\alpha}_{\human}||^2
\end{equation}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
%
%This section introduces the reader to the metric function used herein to address human muscular comfort. 
%This is a crucial element of the proposed system since the planner needs a consistent quantitative assessment of human comfort to be optimized. 
%% 
%% 
%% Inspired in robotics literature, particularly, 
%% in manipulability metrics used to reduce motor torque given a specific end force---see for instance, [#BOOK:1988:Chang], 
%% we seek to assess and evaluate the force generation capabilities of the human arm with regard to their muscle activation level. 
%% 
%% 
%% 
%% 
%In this context, we first take inspiration in robotics literature, particularly, in manipulability metrics used to reduce motor torque given a specific end force---see for instance, \cite{BOOK:1988:Chang,2015_Patel_Tarek_JIRS}.%---where the force manipulability ellipsoid (FME) is usually used 
%
%Force manipulability ellipsoid (FME) is the metric largely used to address such problem, 
%\begin{equation} 
%|| \myvec{\tau} || ^{2} =  \myvec \forcef^{T}\mymatrix J\mymatrix J^{T} \myvec f\leq1,
%\end{equation}
%% 
%where $\mymatrix{J}$ is the geometric Jacobian at a given kinematic configuration. 
%% 
%% 
%% The FME is largely used in robotics literature, but other metrics could also be exploited such as force polytopes \cite{1997_Chiacchio_Vercelli_Pierrot___JRS}
%% which replaces the FME $L_{2}$-norm to an $L_{\infty}$-norm problem
%% with $n$ constraints, where $n$ is the size of $\myvec{\tau}$. 
%% % 
%% Although not being as precise as force polytopes, the FME is more commonly
%% used to optimize the structure of the manipulator workspace \cite{2015_Patel_Tarek_JIRS},
%% and that is due to its reduced number of inequalities and
%% the computational difficulties related to computing the force polytopes\textemdash specifically,
%% transforming the halfspace representation of the polytope vertex \cite{1997_Chiacchio_Vercelli_Pierrot___JRS}. 
%% ===========================================
%% IF WE NEED SPACE:
%% Replace the above text "The FME is largely used....
%% with
%% --------------------------------------------------------------"
%% \footnote{(IF WE NEED TO GAIN SPACE: Replace the text "The FME is largely...") An alternative solution to the FME is the use of force polytopes \cite{1997_Chiacchio_Vercelli_Pierrot___JRS}
%% which replaces the FME $L_{2}$-norm to $n$ constraints based on $L_{\infty}$-norm problem, where $n$ is the size of $\myvec{\tau}$. 
%% Although not being as precise as force polytopes, FME is largely employed in robotics literature and more commonly used due to its computational facilities particularly within optimization \cite{2015_Patel_Tarek_JIRS}.}
%% 
%% "-------------------------------------------------------------
%The force manipulability ellipsoid is efficient in assessing the force generation ability in different directions of the end-pose given a specific joint configuration---more specific, given the Jacobian mapping from end-forces to robot torques. 
%
%Nonetheless, human muscles do not behave linearly to joint torques and are also not symmetric when linking muscular force and torques. 
%Indeed, the FME (as well as other robotics-based manipulability metrics)%
%    \footnote{%
%    FME is largely used in robotics literature due to its computational advantages, particularly for optimization \cite{2015_Patel_Tarek_JIRS}, but other metrics could also be exploited such as force polytopes \cite{1997_Chiacchio_Vercelli_Pierrot___JRS}. 
%} 
% neglects biological motor properties, such as nonlinear joint-torque limitations, and consequently 
%cannot properly assess the force generation capability at the end-pose of a human-arm. 
%
%Herein, we take a different approach and evaluate the muscular comfort optimization problem explicit based on the human muscle activation level required to generate the force for a specific task using the \emph{human force manipulability ellipsoid} (HFME) defined in
%\cite{2015_Tanaka_Nishikawa_Yamada_Tsuji__TransHaptics}. HFME % in \cite{2015_Tanaka_Nishikawa_Yamada_Tsuji__TransHaptics} 
%replaces the torque based pre-image of the unit sphere in the robotics joint space from classic FME to a manipulability based on the 
%human joint torque activation levels $\myvec{\alpha}_{\human}=[\alpha_{1},\dots,\alpha_{7}]^{T}$,
%where $\alpha_{i}\in[0,1]$ represents the activation ratio of the
%$i$-th joint's torque $\tau_{i}$ to its maximum torque $\tau_{i}^{max}$---under maximum voluntary contraction and taking the 
%muscle tension is nearly proportional to the muscle activation level. 
%% 
%
%The resulting torque can be rewritten as a function of $\myvec{\alpha}_\human$, 
%\[ 
%\myvec{\tau}_\human=\mymatrix \Pi (\myvec q_\human, \dot{\myvec q}_\human )\myvec{\alpha}_\human,
%\]
%% % \begin{equation}
%% % \myvec{\tau}_\human=\mymatrix T(\myvec q_\human,\text{sign}\{\dot{\myvec q}_\human\})\myvec{\alpha}_\human,
%% % \label{eq:torque activation level}
%% % \end{equation}
%where 
%% $\mymatrix T(\myvec q_\human,\text{sign}\{\dot{\myvec q}_\human\})$
%$\mymatrix \Pi ( \boldsymbol \cdot )$
%is a diagonal matrix with human maximum torque elements, that is,
%$\text{diag} \{\tau_{1}^{max},\dots,\tau_{7}^{max} \}$. 
%% 
%The matrix $\mymatrix \Pi$
%represents the nonlinear relationship between human torques and joints;
%and each maximum torque element, $\tau_{i}^{max}$, is a nonlinear
%function of the joint values and their directions which is task-dependent. 
%% That is to say the maximum torque for each joint depends not only on its
%% position but also on its derivative (e.g., raising and lowering the
%% upper arm use different muscles). 
%% 
%Experimental data to compute the values for 
%$ \mymatrix \Pi (\myvec q_\human, \dot{\myvec q}_\human ) $
%for different human arm configurations can be found in the excel work of Tanaka et al. \cite{2015_Tanaka_Nishikawa_Yamada_Tsuji__TransHaptics}
%and the values therein are used throughout this work. 
%% Although being
%% computed empirically, values and proportions between joints and maximum
%% torque follows a similar pattern across individuals, even for different
%% body weights whereby results differ only in magnitude, see \cite{2015_Tanaka_Nishikawa_Yamada_Tsuji__TransHaptics}
%% for further details. 
%
%
%Therefore, the explicit expression of the human force manipulability ellipsoid yields 
%\begin{align} 
%\text{HFME}( \myvec q _\human, {^\obj\myvec{f}} , { ^\obj _{\tool} \mymatrix{T} }  )   & 
%          = || \myvec{\alpha}_{\human} || ^{2} 
%          \nonumber
%          \\         & 
%          = \myvec \forcef^{T}\mymatrix   J _\human ( \myvec q _\human )  \mymatrix \Pi ^{-2}  \mymatrix J_\human^{T} ( \myvec q _\human ) \myvec f\leq1,
%          \label{eq : HFME}
%\end{align}
%% 
%where $\mymatrix{J}_\human ( \boldsymbol \cdot ) $  is the geometric Jacobian of the human kinematics at a given $\myvec q _\human$, and 
%$ \myvec f $ is the force in the task-space, that is, the world/robot frame. 
%% 
%
%Note however that the task is defined over the required force in the object frame, that is, $ {^\obj\myvec{f}} $ (which can be straightforwardly mapped to human arm frame $\sum_\human$), and not in the world frame.  
%% 
%For instance, a person drilling a
%board parallel to the floor or to a wall yields different force directions
%in the workspace, but the force direction at the human hand and the board,
%i.e., with respect to $\sum_\human$ and $\sum_\obj$, is the same\textemdash differing
%only by its magnitude. To express the task force (originally described
%in the board frame) in the world frame, we need a spatial transformation from 
%human arm to robot frame. 
%This is achievable by doing a simple adjoint transformation 
%based on $ \myvec q _\human $ and $ { ^\rob _{\obj} \mymatrix{T} }  $, 
%that is, the force in the task-space becomes a function of the human configuration, 
%the frame transformation between human and robot, and the task-dependent force, 
%$ \myvec \forcef ( \myvec q _\human, { ^\rob _{\obj} \mymatrix{T} },  {^\obj\myvec{f}}    ) $. 
%The transformation  is norm-preserving, that is, maintains the same force magnitude, but yields
%different directions which are defined by the arm pose\textemdash and
%consequently by the joint configuration. 
%
%To find (\ref{eq : HFME}), we still need the model of the human arm. 
%% The kinematics and dynamics of a 
%The human limb is often modeled as a
%serial-link kinematic chain with seven degrees of freedom (DOFs) 
%% as shown in Fig. \ref{fig:human robot illustration}
%\textemdash two spherical
%and one revolute joint respectively at the shoulder, wrist and elbow.
%The human to robot arm resemblance enables a direct map from the human
%joint configuration space to the task-space where the force is applied,
%that is, the human-arm forward kinematics 
%% \begin{equation}
%$ 
%\myvec x_\human=\text{FKM}_\human(\myvec q_\human), 
%$  
%% \label{eq:humanHand}
%% \end{equation}
%where $\myvec x_\human$ is the pose of the hand at the point of tool grasping 
%and $\myvec q_\human$ the corresponding joint vector. The differential forward kinematics 
%is then given by $\dot{\myvec x}_\human=\mymatrix J_\human(\myvec q_\human)\dot{\myvec q}_\human$
%where $\mymatrix J_\human( \boldsymbol \cdot )$ is the geometric Jacobian
%of the human arm at a given $\myvec q_\human$ configuration. 
%
%Now, assuming quasi-static movements, the effects of higher order dynamics can be neglected and 
%the end pose force to joint torque mapping depends solely on the exerted interacting force and the gravity effects, that is, 
%\begin{equation}
%\myvec{\tau}_\human  
%             =  \mymatrix J^{T}_\human(\myvec q_\human)  
%                \myvec \forcef ( \myvec q _\human, { ^\rob _{\obj} \mymatrix{T} },  {^\obj\myvec{f}}    ) 
%               + \myvec \rho_\human(\myvec q_\human),
%\label{eq:Final Torque Human}
%\end{equation}
%where $\myvec \rho \human$ represent the vector of the gravity force. 
%               
%Herein, the gravitational forces results from the contribution of the upper arm and forearm weights and center of mass, and the tool mass and distance to the end pose. Naturally, the gravitational forces are well-defined in the inertial frame and do not depend on the arm configuration. However their gravitational torque---respectively, over the shoulder, shoulder and elbow system and for the full arm---depends on the joint configuration. 
%
%Taking the human modeling, we can update the HFME accordingly, that is, combining (\ref{eq : HFME}) and (\ref{eq:Final Torque Human}), 
%\begin{align} 
%\text{HFME} & ( \myvec q _\human, { _{\obj} \mymatrix{T} },  {^\obj\myvec{f}} , { ^\obj _{\tool} \mymatrix{T} }  ) = 
%                        ( \mymatrix J^{T} \myvec \forcef  + \myvec \rho_\human )^T \Pi ^{-2} ( \mymatrix J^{T} \myvec \forcef  + \myvec \rho_\human ). 
%%           \nonumber
%%           \\         & 
%%           = ( \myvec \forcef ( \myvec q _\human, { ^\rob _{\obj} \mymatrix{T} },  {^\obj\myvec{f}}    )    J _\human ( \myvec q _\human ) 
%%              + \myvec \rho_\human(\myvec q_\human) 
%%             )^T
%%  \mymatrix \Pi ^{-2}  \mymatrix J_\human^{T} ( \myvec q _\human ) \myvec f\leq1,
%          \label{eq : HFME Final}
%\end{align}
%Function arguments in the right side of the equation have been removed to improve readability, but note that all terms 
%% in $ ( \mymatrix J^{T} \myvec \forcef  + \myvec \rho_\human ) $ 
%depend on the $ \myvec q _\human $, and $ \myvec \forcef $ also depends on $ { ^\rob _{\obj} \mymatrix{T} }$ and ${^\obj\myvec{f}} $. 
%
%
%
%From the resulting HFME  (\ref{eq : HFME Final}), we can describe the muscular comfort function to be maximized as 
%\begin{equation}
% \text{Muscular} ( \myvec q _\human, { _{\obj} \mymatrix{T} },  {^\obj\myvec{f}} , { ^\obj _{\tool} \mymatrix{T} }  ) = 1 / \text{HFME}. 
%\end{equation}
%Note that HFME is defined over the $L_{2}$-norm of the muscle activation level $\myvec{\alpha}_{\human}$ which is naturally upper-bounded by $1$. 
%
%
%% 
%% 
%
%
%
%
%
%
%
%
%
%
%
%
%


==> New folder/Conclusion/Conclusion.tex <==
\section{Conclusion and Future Work}

%<<<<<<< .mine
%We have proposed an optimization based planner to grasp and position an object
%for a human applying forceful operations on the object.  The planner considers
%the muscular and peripersonal-space comfort metrics proposed in this paper.
%Based on the results, our future work will focus on (i) improving the
%peripersonal-space metric to better represent human perception, (ii) improving
%the planning time to enable fluent human interaction on continuous forceful
%tasks, and (iii) adding other metrics to our framework, e.g. metrics that take
%into account the visibility of the task execution by the human.
%=======
This work 
proposed a new technique for grasp planning and object positioning that explicitly concerns human configuration, safety and comfort. 
To this aim, we developed a new criteria to cope with both muscular comfort and safety perception 
in a quantiative manner which allowed us to analyze the desired comfort without having to rely on experience and intuition alone. 
For the muscular comfort, 
the proposed planner succed in minimizing the 
human joint-torque muscular activation level required to execute a given forceful task, 
whilst human safety perception was addressed through the optimization of the subject peripersonal space 
and distance during HRI. 
Both criteria were optimized taking human-robot kinematic constraints and ensuring safe and stable grasping from the robotic counterpart. 
Validity and effectiveness of our algorithm were first analyzed through different simulation scenarios and then 
validated with different human-robot experiments. The results highlighted the effectiveness of the proposed planner 
and the necessity to explicitly consider and plan for the human and not only for the task. 
Based on the results, our future work will focus on (i) improving the
peripersonal-space metric to better represent human perception, (ii) improving
the planning time to enable fluent human interaction on continuous forceful
tasks, and (iii) adding other metrics to our framework, e.g. metrics that take
into account the visibility of the task execution by the human.

%>>>>>>> .r325

%<<<<<<< .mine
%motion--easy for human to move
%
%singularity--robot motion, avoid singularity
%
%visibility
%=======


% motion--easy for human to move
% 
% singularity--robot motion, avoid singularity
% 
% visibility>>>>>>> .r325


==> New folder/Experiment/Experiment.tex <==
\section{Experiments and results}
\label{sec:Experiments} 

We implemented the comfort metrics, the stability check, and the optimization
process in Python.  We used the Baxter robot from Rethink Robotics and OpenRAVE (openrave.org)
%\cite{diankov2008openrave} 
for forward/inverse-kinematic calculations for the
human and robot model.  We used the SciPy library for optimization,
particularly the SLSQP
implementation\footnote{https://docs.scipy.org/doc/scipy/reference/optimize.minimize-slsqp.html}.
We used 64 points distributed around the whole body model of the human and 56
points for the whole body of the robot to compute the peripersonal-space
metric. We weighted the muscular and peripersonal space comfort equally during the optimization, 
yet it is worth noting that different weighting schemes may be chosen accordinglying to a given task and human preferences, e.g., their priors on HRI.
%A proper way to determine the weight scheme is trying different combinations in human experiments and then identifying the one with more human preference. } 

We consider two tasks. First, the task of cutting a circle out of a foam board.
We divided the circle into 16 discrete points
(Fig.~\ref{fig:comfortcurveData}). We call the application of the cutting force
on one of these 16 points a cutting operation; i.e. the discrete points along
the circle give us 16 different cutting operations.
%We used each forceful cutting position and
%direction on these 16 points as a forceful cutting operation. 
The force
direction was aligned with the cutting direction. Using a force-torque sensor
we estimated the force required for cutting into foam as 30N. The second task
is the drilling task. 
We identified 9 points uniformly distributed on a foam
board in a 3-by-3 grid. 
We call the application of the drilling force on one of these 9 points a drilling operation.
The force direction was taken normal and into the
board. Using a force-torque sensor we estimated the force for drilling into the
foam as 15N. 


%This section presents experimental assessment of the proposed human-comfort based planner in multiple scenarios---both in simulated and in real robot experiments% 
%\footnote{For the simulations, we used OpenRAVE environment \cite{diankov2008openrave}, 
%whilst experiments were devised using the Baxter robot from Rethink Robotics, a 7-DOF bimanual manipulator equipped with parallel jaw grippers.}.  
%In all experiments, we assume the information regarding human/robot kinematics and transformation frame is made available. 
%Also, we assume a fixed grasp between the human and the tool as discussed in Sec.~\ref{sec:defi}---the grasping for drilling and cutting applications assessed herein is shown in Fig.~\ref{fig:hand-tool}.  
%
%Our goal in this Section is to investigate 
%(i) the efficiency of the muscular comfort in assessing different muscle activation levels at different configurations, 
%(ii) the consistency and efficiency of the algorithm to cope with both muscle and peripersonal metrics, 
%and, finally,
%(iii) to analyze human perception with regard to the predicted metric and proposed configuration given by our planner. 





% 
% \begin{figure}[thpb]
% 	\begin{center}
% 		\mbox{
% 			\subfigure[cutting]{{
% 					\label{fig:subfig:cutting}  
% 					\includegraphics[width=1.6 in, angle=-0]{Experiment/fig/cutting}}}
% 			
% 			\subfigure[drilling]{{
% 					\label{fig:subfig:drilling}  
% 					\includegraphics[width=1.6 in, angle=-0]{Experiment/fig/drilling}}}		
% 		}
% 		
% 		\caption{Two forceful tasks in the experiments.}
% 		\label{fig:tasks}
% 	\end{center}
% \end{figure}
% 


%\begin{figure}[thpb]
%	\begin{center}
%		\mbox{
%			\subfigure[Grasping a cutter]{{
%					\label{fig:subfig:circulaut1}  
%					\includegraphics[width=1.6 in, angle=-0]{Experiment/fig/hand_cut}}}
%			
%			\subfigure[Grasping a drill]{{
%					\label{fig:subfig:circularc5}  
%					\includegraphics[width=1.6 in, angle=-0]{Experiment/fig/hand_drill}}}		
%		}
%		
%		\caption{Human grasp configurations of tools. }
%		\label{fig:hand-tool}
%	\end{center}
%\end{figure}




\subsection{Analysis of the Muscular Comfort Metric}

First, to better understand and validate the proposed muscular comfort metric
we compared its predictions with known comfortable and uncomfortable configurations. 
%We want to qualitatively analyze if the muscular comfort function is able to cope with them 
%and if the measures coincide with our perception of physical comfort when a human performs a forceful operation. 

Take for example, the task of cutting off a circular piece of a board, as shown in Figs.~\ref{fig:subfig:cut5good} and \ref{fig:subfig:cut5bad}. 
From the task definition, we expect fluctuations of muscular comfort at different configurations---from comfortable to very uncomfortable ones.  
Particularly, configurations at the proximity of joint limits, specially at the wrist spherical joint, 
are known to be very uncomfortable and have less force generation capabilities. 

%
\begin{figure}[!t]
	\centering
	\includegraphics[width=3.4in, angle=-0]{Experiment/fig/comfortcurve}
    \caption{Muscular comfort values for different cutting points along a circle. The circled letters on the graph correspond to the configurations in Fig.~\ref{fig:comfortcurve}.
    %with arm configurations. The point on the dark orange curve depicts the value of muscular comfort when human poses at the most comfortable configuration. The point on the light orange curve represents the value of muscular comfort when human poses at the most uncomfortable configuration.
    }
	\label{fig:comfortcurveData}
\end{figure}

%In the scenario, a human is required to cut off a circular piece from the board
%using a cutter held by his right hand as shown in Fig.~\ref{fig:comfortcurve}.
%The continuous force (constant with respect to the hand or the tool, but moving
%along the cutting direction, that is, along the object frame) defines the task.
%For the sake of simplification, we sample a set of 16 operations to represent
%the continuous cutting task. 
For each of the 16 discretized points along the circle, we computed a set of
feasible inverse-kinematics (IK) solutions for the human to perform the
forceful operation at that point. Then we computed the corresponding muscular
comfort values for all the IK solutions.
We present the computed muscular comfort values in Fig.~\ref{fig:comfortcurveData}. 
The dark orange curve depicts the change of muscular comfort when human is at the most comfortable configuration for a cutting operation, whilst the light orange depicts the worst (most uncomfortable) configuration for that cutting point. 
The range of possible human choices, illustrated in Fig.~\ref{fig:comfortcurve}, coincides with the human arm redundancy stressed in Sec.~\ref{sec:defi}. 
For the two possible configurations in Fig.~\ref{fig:comfortcurve}, our experience is that configuration \textcircled{{\small a}} is much more comfortable than configuration \textcircled{{\small b}}, which coincides with the results based on the muscular comfort metric.
%Since we assuming the hypothesis that humans will choose the most comfortable configuration, we will focus on the most comfortable configuration. 



\begin{figure}[!t]
	\centering
	%\framebox{\parbox{3in}{We suggest that you use a text box to insert a graphic (which is ideally a 300 dpi TIFF or EPS file, with all fonts embedded) because, in an document, this method is somewhat more stable than directly inserting a picture.
	%}}
	\mbox{
		\subfigure[config.{\small  \textcircled{a}}]{{
				\label{fig:subfig:cut5good}  
				\includegraphics[width=1.3 in, angle=-0]{Experiment/fig/_circularcut5good}}}
		
		\subfigure[config.{\small  \textcircled{b}}]{{
				\label{fig:subfig:cut5bad}  
				\includegraphics[width=1.3 in, angle=-0]{Experiment/fig/_circularcut5bad}}}	
	}
    \caption{Two different arm postures while cutting the top of the board with different muscle comfort performance (see force position $f_5$ in Fig.~\ref{fig:comfortcurveData} with muscular comfort values {\small  \textcircled{a}} and {\small  \textcircled{b}}). }
% 	The change of muscular comfort for a circular cutting task. (a) and (b) snapshot two configurations in accordance with values in the curve. }
	\label{fig:comfortcurve}
\end{figure}


%From the most comfortable curve in Fig.~\ref{fig:comfortcurveData}, we can also straightforwardly observe that different cutting configurations---requiring different arm postures---generated different muscle comfort measures, as expected. 
%This is crucial since if the metric weren't able to differentiate the variety of configurations presented in this task, 
%it would imply a reduced applicability. 

At the proximity of joint limits shown in force position $f_{10}$ (positions $f_{11}$
and $f_{12}$ are not feasible due to joint limits), we can see a degradation in muscular
comfort and that the range of possible comfort values is narrower (due to the possible loss of a DoF). 
%This
%posture is illustrated in Fig.~\ref{fig:subfig:circularcut5}, configuration
%\textcircled{{\small d}}.  
Finally, we can also see consistency in result at
the point of circular closing (force positions 16 to 1)
%---illustrated in
%configuration \textcircled{{\small a}}  and \textcircled{{\small f}}. 
%The
%muscular comfort analysis in Fig.~\ref{fig:comfortcurveData} shows similar
%performance as expected. 

Fig.~\ref{fig:comfortcurveData} also shows us that it is critical to plan
optimal robot and object configurations to perform comfortable human-robot
collaboration. For example, for the circular-cutting task, if a robot keeps
rotating the object to enable the human configuration in
Fig.~\ref{fig:subfig:cut5good}, the required muscular effort for the human can
stay low during the cutting of the whole circle.

%\begin{figure}[!t]
%	\begin{center}
%		\mbox{
%			\subfigure[config.{\small{\textcircled{a}}}]{{
%					\label{fig:subfig:circularcut1}  
%					\includegraphics[width=1.6 in, angle=-0]{Experiment/fig/_circularcut1}}}
%			
%			\subfigure[config.{\small  \textcircled{d}}]{{
%					\label{fig:subfig:circularcut5}  
%					\includegraphics[width=1.6 in, angle=-0]{Experiment/fig/_circularcut10}}}		
%		}
%		
%		\mbox{
%			\subfigure[config.{\textcircled{e}}]{{
%					\label{fig:subfig:circularcut10}  
%					\includegraphics[width=1.6 in, angle=-0]{Experiment/fig/_circularcut13}}}
%			\subfigure[config.{\small  \textcircled{f}}]{{
%					\label{fig:subfig:circularcut16}  
%					\includegraphics[width=1.6 in, angle=-0]{Experiment/fig/_circularcut16}}}			
%		}		
%        \caption{Comfortable human configurations for the circular cutting. Circled letters correspond to configurations shown in Fig.~\ref{fig:comfortcurveData}}
%		\label{fig:circularcut}
%	\end{center}
%\end{figure}


\subsection{Optimization performance: Simulation}

We evaluated the performance of the combined optimization of our comfort metrics by comparing it to other planners.
We implemented four planners:
\begin{itemize}
    \item{Comfort planner}: Our planner optimizing both metrics.
    \item{Random planner}: Given a forceful operation, the random planner randomly picks an object pose within the reachable space of the robot. Then it searches one feasible robot configuration in terms of static stability, and then chooses the optimized human configuration in terms of both muscular and peripersonal comfort under the constraint of human reachability to perform the task. The planner acts as baseline.
    \item{Muscular planner}: The muscular planner only takes the muscular comfort as cost (i.e., $w_\text{P}=0$ in Eq.~\ref{most}).
       % to optimize robot and object configurations and provide reference human configuration $(\textbf{\textit{q}}_{\text{h}},\, _{\text{h}}^{\text{}}\textbf{\textit{T}})$ which is comfortable in terms of muscular comfort;
    \item{Peripersonal planner}: Similarly, the planner just maximizes the human's peripersonal comfort  (i.e., $w_\text{M}=0$).
       % to produce comfortable robot and object configurations for the operation. 	 
\end{itemize}


%In this section, we devise multiple drilling and cutting operations (16 and 9, respectively) at different points in a board. 
%We want to analyze consistency of the algorithm, that is, if it is able to cope with all tasks simulated multiple times in a consistent manner, 
%and 
%efficiency, that is, if it able to provide good results for both muscular and peripersonal metrics. 
%To analyze efficiency, we compared our planner (we call it \textit{comfort} planner for distinguishing), with another three planners, i.e., \textit{random} planner, \textit{muscular} planner and  \textit{peripersonal} planner. 
%Given a forceful operation $(^\text{o}\textbf{\textit{f}},\, _{\text{t}}^{\text{o}}{\textbf{\textit{T}}})$,
%\begin{itemize}
%	\item{Random planner}: 
%	the random planner randomly picks the first feasible robot and object configuration $(\textbf{\textit{q}}_{\text{r}},\, _{\text{o}}\textbf{\textit{T}})$ in terms of quasi-statical equilibrium and geometrical accessibility for the robot, and then chooses the optimized human configuration $(\textbf{\textit{q}}_{\text{h}},\, _{\text{h}}^{\text{}}\textbf{\textit{T}})$ in terms of both muscular and peripersonal comfort under the constraint of human reachability to perform the task. The planner acts as baseline approach;
%	\item{Muscular planner}:
%	the muscular planner only take the muscular comfort as the cost (i.e., $w_\text{P}=0$ in Equation~\ref{most}) to optimize robot and object configurations and provide reference human configuration $(\textbf{\textit{q}}_{\text{h}},\, _{\text{h}}^{\text{}}\textbf{\textit{T}})$ which is comfortable in terms of muscular comfort;
%	\item{Peripersonal planner}: similarly, the planner just maximizes the human's peripersonal comfort  (i.e., $w_\text{M}=0$ in Equation~\ref{most}) to produce comfortable robot and object configurations for the operation. 	 
%\end{itemize}

\begin{table*}[]
	\centering
\caption{Average comfort results of four planners on 16 cutting and 9 drilling operations. Normalized with Random Planner results. 
    %Musc. comfort values are normalized using the musc. comfort value of random planner. Similarly for peripersonal-space comfort. 
Larger value is more comfort.} 
%The symbol $A\tfrac{\text{B}}{\text{C}}$ represents $A^{\text{B}}/A^{\text{C}}$. }
	\label{table:average}
	\begin{tabular}{@{}ccccccccc@{}}
		\toprule
		& \multicolumn{2}{c}{Random Planner} & \multicolumn{2}{c}{Comfort Planner}  & \multicolumn{2}{c}{Peripersonal Planner} & \multicolumn{2}{c}{Muscular Planner} \\ \cmidrule(l){2-3} \cmidrule(l){4-5} \cmidrule(l){6-7} \cmidrule(l){8-9} 
		%& $M\tfrac{\text{R}}{\text{R}}$       & $P\tfrac{\text{R}}{\text{R}}$     & $M\tfrac{\text{C}}{\text{R}}$     & $P\tfrac{\text{C}}{\text{R}}$      & $M\tfrac{\text{P}}{\text{R}}$        & $P\tfrac{\text{P}}{\text{R}}$        & $M\tfrac{\text{M}}{\text{R}}$      & $P\tfrac{\text{M}}{\text{R}}$      \\ \midrule
		& Musc. Comf.      & Perip. Comf.    & Musc. Comf.    & Perip. Comf.     & Musc. Comf.       & Perip. Comf.       & Musc. Comf.     & Perip. Comf.     \\ \midrule
		Cutting  & 1             & 1           & 11.19  & 2.08 & 0.34  & \textbf{2.09 }& \textbf{15.66}  & 1.02   \\
		Drilling & 1             & 1           & 19.24 & \textbf{2.55} & 5.78   & 2.51 & \textbf{22.45 } & 0.94  \\ \bottomrule
	\end{tabular}
\end{table*}


%\begin{table*}[]
%	\centering
%	\caption{Average results of four planners on a cutting and a drilling operation. All results are normalized using the results of random planner. The little a value is, the better its corresponding performance is.  }
%	\label{table:average}
%	\begin{tabular}{@{}ccccccccc@{}}
%		\toprule
%		& \multicolumn{2}{c}{Random Planner} & \multicolumn{2}{c}{Comfort Planner}  & \multicolumn{2}{c}{Peripersonal Planner} & \multicolumn{2}{c}{Muscular Planner} \\ \cmidrule(l){2-9} 
%		& $M^R/M^R$       & $P^R/P^R$      & $M^C/M^R$      & $P^R/P^C$      & $M^P/M^R$        & $P^R/P^P$       & $M^M/M^R$        & $P^R/P^M$       \\ \midrule
%		cutting  & 1             & 1           & 0.174211802 & 0.489449784 & 3.557843  & \textbf{0.486476059 }& \textbf{0.12384735}  & 0.920642799   \\
%		drilling & 1             & 1           & 0.008512361 & \textbf{0.413836036} & 0.828656189   & 0.421266784 & \textbf{0.00743559 } & 0.739188149  \\ \bottomrule
%	\end{tabular}
%\end{table*}
We ran all our planners on the 25 operations (16 cutting and 9 drilling).
Table~\ref{table:average} shows the average results of the four planners for both cutting and drilling operations.
%---note that the muscular comfort is denoted by $M^\text{R}$, whilst the peripersonal comfort is described by $P^\text{R}$. 
% as discussed in Fig.~\ref{fig:tasks}. 
%For the sake of simplicity and to 
To improve readability, results from the random planner were used as baseline to normalize the results of other planners:
For each task (drilling and cutting), muscular comfort values are normalized using the muscular comfort value of Random Planner. Similarly for the peripersonal-space comfort values.

As expected, the Peripersonal Planner outperforms others for peripersonal comfort (improvement of $2.09$ times over the random planner), yet it performs poorly ($0.34$ of the random planner) when it comes to muscular comfort. 
%The muscular comfort was only $0.34$ of the random planner---being the worst result. 
The muscular planner has similar performance: it outperforms for muscular comfort but performs poorly when considering peripersonal comfort. 
In constrast to other planners, the proposed Comfort Planner is able to optimize both metrics close to the values achieved by the planners optimizing individual metrics.
This highlights that it is possible to cope with both muscular and peripersonal comfort without much compromise.  


% 
% As shown in the table, for the cutting task, on average, the peripersonal planner performs best in terms of maximizing the peripersonal comfort (2.09 times larger than random planner) but the average muscular comfort (0.34) is quite small compared with the results (1/11.19/15.66) of other planners, which indicates the necessity of integrated optimization. Similarly,
% the muscular planner achieves the maximum muscular comfort (15.66 times) among the four planners, but its average peripersonal comfort (1.02 times) is not well optimized compared with the other two planners (2.08/2.09). 
% 
% Instead, the comfort planner shows impressive performance in maximizing both muscular comfort (11.19 times) and peripersonal comfort (2.08 times). Similar results were seen for the drilling operations. Still, the comfort planner stands out in planning comfortable configurations in terms of both muscular comfort (1/\textbf{19.24}/5.78/22.45/) and peripersonal comfort (1/\textbf{2.55}/2.51/0.94).

We present configurations found by the planners for one cutting operation
in Fig.~\ref{fig:cut_optimizationresults} and for one drilling operation in
Fig.~\ref{fig:drill_optimizationresults}. Again, we see that the Comfort
Planner can generate solutions that are comfortable according to
both metrics.

We realized that a limitation of the proposed implementation is the time it takes to generate results.
To compute one configuration, the Comfort Planner took 9.4 seconds on average over the 25 operations, with a standard deviation of
1.8. Most of this time was spent on generating
IK solutions. These time results indicate that faster schemes
must be developed if the robot is to perform fluent interaction with a human
during a continuous task. We are currently investigating methods based on
precomputing IK solutions.

%illustrates the planning results for one cutting operation. As shown in Fig.~\ref{fig:subfig:random-cut}, the random planner requires the human to stand close behind the robot and perform the cutting at a high altitude. Obviously, the configuration is far from comfortable for the human operator. The results of muscular planner (Fig.~\ref{fig:subfig:muscular-cut}) and peripersonal planner (Fig.~\ref{fig:subfig:safety-cut}) show excellences in terms of reducing muscular discomfort and peripersonal discomfort respectively. But still, they are still not entirely comfortable and even visibly uncomfortable. For example, the configuration in Fig.~\ref{fig:subfig:muscular-cut} positions the human and the robot at a very close distance, while the configuration in Fig.~\ref{fig:subfig:safety-cut} requires the human to fully extend his arm but apply a large cutting force. The solution in Fig.~\ref{fig:subfig:comfort-cut} leaves sufficient room between the human and the robot, and allows the human to perform the operation at a flexible configuration.
%Similarly in Fig.\ref{fig:drill_optimizationresults}, for one of the the 9 drilling operations, the random planner produces configurations with considerable muscular discomfort and peripersonal discomfort as shown in  Fig.~\ref{fig:subfig:random-drill}. Still, the muscular planner (Fig.~\ref{fig:subfig:muscular-drill}) and perpesonal planner (Fig.~\ref{fig:subfig:safety-drill}) performs well in maximizing muscular and perpersonal comfort respectively, while the comfort planner provide an solution (Fig.~\ref{fig:subfig:comfort-drill}) which is comfortable from both aspects. 


\begin{figure*}[!thpb]
	\begin{center}
		\mbox{
			
            \subfigure[Random Planner]{{%: ${M=8.34,\,P=20.43}$]{{
					\label{fig:subfig:random-cut}  
					\includegraphics[width=1.6 in, angle=-0]{Experiment/fig/1cut_randomer}}}
				
                    \subfigure[Comfort planner]{{%: ${M^{\text{C}}=47.10,\,P^{\text{C}}=43.30}$]{{
		\label{fig:subfig:comfort-cut}  
		\includegraphics[width=1.6 in, angle=-0]{Experiment/fig/1cut_optimizer}}}								
        \subfigure[Muscular planner]{{%: ${M^{\text{M}}=48.53,\,P^{\text{M}}=23.38}$]{{
					\label{fig:subfig:muscular-cut}  
					\includegraphics[width=1.6 in, angle=-0]{Experiment/fig/1cut_comforter}}}		
			
                    \subfigure[Peripersonal planner]{{%: ${M^{\text{P}}=3.98,\,P^{\text{P}}=44.23}$]{{
					\label{fig:subfig:safety-cut}  
					\includegraphics[width=1.6 in, angle=-0]{Experiment/fig/1cut_safetyer}}}						

		}
		
        \caption{Optimization results for a cutting operation. The comfort values are: 
        (a) Musc. comfort: 8.34; Perip. comfort: 20.43.
        (b) Musc. comfort: 47.10; Perip. comfort: 43.30.
        (c) Musc. comfort: 48.53; Perip. comfort: 23.38.
        (d) Musc. comfort: 3.98; Perip. comfort: 44.23.
         }
		\label{fig:cut_optimizationresults}
	\end{center}
    \vspace{-3mm}
\end{figure*}


\begin{figure*}[!thpb]
	\begin{center}
		\mbox{
            \subfigure[Random planner]{{
            %, ${M^{\text{R}}=3.70,\,P^{\text{R}}=20.21}$]{{
					\label{fig:subfig:random-drill} 
					\includegraphics[width=1.65 in, angle=-0]{Experiment/fig/1drill_randomer}}}
                    \subfigure[Comfort planner]{{%, ${M^{\text{C}}=59.19,\,P^{\text{C}}=44.75}$]{{
		\label{fig:subfig:comfort-drill}  
		\includegraphics[width=1.6 in, angle=-0]{Experiment/fig/1drill_optimizer}}}	

        \subfigure[Muscular planner]{{%, ${M^{\text{M}}=42.33,\,P^{\text{M}}=21.88}$]{{
					\label{fig:subfig:muscular-drill}  
					\includegraphics[width=1.6 in, angle=-0]{Experiment/fig/1drill_comforter}}}		
			
                    \subfigure[Peripersonal planner]{{%, ${M^{\text{P}}=4.72,\,P^{\text{P}}=44.40}$]{{
					\label{fig:subfig:safety-drill}  
					\includegraphics[width=1.6 in, angle=-0]{Experiment/fig/1drill_safetyer}}}					
		
		}		
		\caption{Optimization results for a drilling operation. The comfort values are:
        (a) Musc. comfort: 3.70; Perip. comfort: 20.21.
        (b) Musc. comfort: 59.19; Perip. comfort: 44.75.
        (c) Musc. comfort: 42.33; Perip. comfort: 21.88.
        (d) Musc. comfort: 4.72; Perip. comfort: 44.40.
    }
		\label{fig:drill_optimizationresults}
	\end{center}
\end{figure*}


%% Please add the following required packages to your document preamble:
%% \usepackage{booktabs}
%\begin{table*}[]
%	\centering
%	\caption{Optimization results of four planners on 9 drilling operations.}
%	\label{table:drilling} 
%	\begin{tabular}{@{}ccccccccc@{}}
%		\toprule
%& \multicolumn{2}{c}{random} & \multicolumn{2}{c}{comfort}  & \multicolumn{2}{c}{peripersonal-space} & \multicolumn{2}{c}{muscular} \\ \cmidrule(l){2-9} 
%& $c_M^R/c_M^R$       & $d^R/d_P^R$      & $c_M^C/c_M^R$      & $d^R/d^C$      & $c_M^P/c_M^R$        & $d^R/d^P$       & $c_M^M/c_M^R$        & $d^R/d_P^M$       \\ \midrule
%		0 & 1            & 1           & 0.008209705 & 0.384008672 & 1.146243546  & 0.417541259 & 0.008327502   & 0.484730845  \\
%		1 & 1            & 1           & 0.001586443 & 0.543418801 & 0.224394093  & 0.559807953 & 0.001184157   & 0.826631458  \\
%		2 & 1            & 1           & 0.012860702 & 0.241515079 & 0.048389127  & 0.277322702 & 0.011396077   & 0.41805713   \\
%		3 & 1            & 1           & 0.005828652 & 0.425407424 & 0.265862803  & 0.442944871 & 0.007440348   & 0.926383168  \\
%		4 & 1            & 1           & 0.008390956 & 0.424619962 & 0.985386118  & 0.443660158 & 0.006601949   & 0.550746649  \\
%		5 & 1            & 1           & 0.0062740607  & 0.4515184135 & 0.0794475515  & 0.4550742458 & 0.0079809251  & 0.9234282501  \\
%		6 & 1            & 1           & 0.003575723 & 0.47864771  & 4.216434141  & 0.482909299 & 0.002811497   & 0.542906355  \\
%		7 & 1            & 1           & 0.021980698 & 0.309683394 & 0.203253628  & 0.339464507 & 0.013271584   & 0.34995709   \\
%		8 & 1            & 1           & 0.007904312 & 0.465704872 & 0.288494696  & 0.520782314 & 0.007906267   & 0.591002571  \\ \bottomrule
%	\end{tabular}
%\end{table*}
%
%% Please add the following required packages to your document preamble:
%% \usepackage{booktabs}
%% \usepackage{multirow}
%\begin{table*}[]
%	\centering
%	\caption{Optimization results of four planners on 16 cutting operations.}
%	\label{table:cutting} 
%	\begin{tabular}{@{}ccccccccc@{}}
%		\toprule
%& \multicolumn{2}{c}{random} & \multicolumn{2}{c}{comfort}  & \multicolumn{2}{c}{peripersonal-space} & \multicolumn{2}{c}{muscular} \\ \cmidrule(l){2-9} 
%& $c_M^R/c_M^R$       & $d^R/d_P^R$      & $c_M^C/c_M^R$      & $d^R/d^C$      & $c_M^P/c_M^R$        & $d^R/d^P$       & $c_M^M/c_M^R$        & $d^R/d_P^M$       \\ \midrule
%		0                  & 1            & 1            & 0.169343505 & 0.4720148453 & 2.71028196       & 0.462021294      & 0.170998224       & 0.874235986       \\
%		1                  & 1            & 1            & 0.305869151 & 0.479056288 & 2.415038179       & 0.497886643      & 0.078025614       & 0.770591899       \\
%		2                  & 1            & 1            & 0.637361865 & 0.635978061 & 4.953041713       & 0.608171482      & 0.189692005       & 0.943988839       \\
%		3                  & 1            & 1            & 0.296490719 & 0.522672516 & 3.667184171       & 0.463887972      & 0.29694739        & 1.072374915       \\
%		4                  & 1            & 1            & 0.052149227 & 0.463227546 & 2.431252902       & 0.487102791      & 0.014308077       & 0.757360952       \\
%		5                  & 1            & 1            & 0.024971972 & 0.458809896 & 1.549858371       & 0.446361385      & 0.050851005       & 0.603481237       \\
%		6                  & 1            & 1            & 0.06721818  & 0.531334461 & 2.226083819       & 0.529049648      & 0.06384763        & 1.032690145       \\
%		7                  & 1            & 1            & 0.186219251 & 0.5442705   & 6.389876656       & 0.505424986      & 0.143214271       & 1.017694347       \\
%		8                  & 1            & 1            & 0.045957041 & 0.444784215 & 3.633729511       & 0.451922838      & 0.026778045       & 0.804862547       \\
%		9                  & 1            & 1            & 0.07440223  & 0.394526522 & 3.048161463       & 0.471640153      & 0.067748427       & 0.78264381        \\
%		10                 & 1            & 1            & 0.261078947 & 0.497680699 & 6.733899069       & 0.538839047      & 0.370031137       & 1.25503871        \\
%		11                 & 1            & 1            & 0.074823619 & 0.640346868 & 3.99855008        & 0.592330666      & 0.074831674       & 1.27502901        \\
%		12                 & 1            & 1            & 0.113059934 & 0.506585967 & 1.731853307       & 0.474957347      & 0.078498154       & 0.876644428       \\
%		13                 & 1            & 1            & 0.069507089 & 0.369449929 & 1.870946614       & 0.363621684      & 0.06340036        & 0.750020258       \\
%		14                 & 1            & 1            & 0.183264954 & 0.337557155 & 5.860910836       & 0.365935609      & 0.177048672       & 0.684456702       \\
%		15                 & 1            & 1            & 0.225671146 & 0.532901082 & 3.70482574        & 0.524463405      & 0.115338279       & 1.229171          \\ \bottomrule
%	\end{tabular}
%\end{table*}
%
%
%\begin{figure*}[thpb]
%	\begin{center}
%		\mbox{	
%			\subfigure[gripper placement/missing]{{
%					\label{fig:subfig:gripper}  
%					\includegraphics[width=2.1 in, angle=-0]{Experiment/fig/weightedsum}}}			
%			
%			\subfigure[sum weighted min]{{
%					\label{fig:subfig:weightedsum}  
%					\includegraphics[width=2.1 in, angle=-0]{Experiment/fig/weightedsum}}}
%			\subfigure[sum min]{{
%					\label{fig:subfig:topweightedsum}  
%					\includegraphics[width=2.1 in, angle=-0]{Experiment/fig/maxmin}}}			
%		}
%		
%		\caption{optimization with different safety schemes.}
%		\label{fig:safetyschemes}
%	\end{center}
%\end{figure*}
%




\subsection{Human experiments}

Finally, 
we conducted a series of human-robot experiments to evaluate human experience and comfort perception 
during a forceful operation with real cooperative robot. 

%We decided for using the Baxter robot from Rethink Robotics as the robot platform due to its compliance capabilities 
%and, most important, by its easy to use 
The Baxter robot 
gravity compensation mode is activated by a sensor at the arms cuff on which participants could easily hold.
Using this feature, $5$ participants were asked to engage in motion activities with the Baxter robot in order to familiarize themselves with the robot and to improve their psychological comfort.
The participants were also briefed about the goal of the study and the tasks they were expected to perform. 

The tasks required were three pairs of drilling and cutting on a foam board tightly held by the Baxter robot. 
First, (i) the participants were asked to move the robot arms using the gravity compensation mode
%\footnote{The gravity compensation mode from the Baxter was also used in the first part of the study.} 
to a position they felt comfortable and safe to interact, and drill through the center of a foam board; 
then (ii) they were asked to do the same but for a cutting operation. 
We then moved the Baxter arms to previously set configurations which were randomly obtained (one for drilling and another one for cutting operations). 
Participants were then asked to (iii) drill and then (iv) cut the board at random robot configurations. 
Finally, 
we moved the Baxter arms to previously decided configurations 
based on our Comfort Planner 
(one optimized robot configuration for drilling and another one for cutting). 
Participants were then asked to (v) drill and (vi) cut at the optimized configurations. 
Some of these operations are shown in Fig.~\ref{fig:realExperiments}. 



%For tasks (iii) to (vi), 
%participants were also instructed to follow the specific arm postures suggested by our planner, reducing their flexibility over the redundant space. 
%We then asked them to use self-motion (mostly the redundancy over the elbow) to try to find a better posture to execute the tasks. 
%This experiment analysis has been devised to investigate our hypothesis of choosing the best human posture among the redundant space---stressed in Sec.~\ref{sec:defi}.   
%Among the five participants, only one could find a better configuration for the drilling tasks (iii) and (v), but he/she also exploited the drilling task redundancy, that is, the drill can rotate within the drilling axis; but none of the participants were able to find a better arm posture for cutting the board at the specific configuration previously set by the robot. 
%

After the experiments, for each scenario, 
participants were asked to grade from 1 to 10 (higher better), their perception on the human-robot safety and peripersonal comfort, and their perception over the muscular forces demanded during the task execution. %, that is, their perception on the muscular comfort.  
The scores are summarized in Fig.~\ref{fig:baxter results:safety} for peripersonal comfort and in Fig.~\ref{fig:baxter results:comfort} for muscular comfort. 
%In the left of each figure, readers can see the drilling operation for user defined object pose, for the operation based on random planner, and user operation based on our optimized human comfort based planner (in this order), whilst the cutting operation results are shown in right. 
From both figures, it is easy to see participants perception regarding the peripersonal and muscular comfort agrees with our expectations, particularly for the drilling operation. 
Cutting operation was clearly not as comfortable as drilling---even for participants' own choice of object positioning. 
Significant difference between the Random Planner and the Comfort Planner is seen for the muscular comfort perception for the drilling operation. %This particular result also highlights the importance to explicitly consider and plan for the human comfort during interaction, which is crucial to foster real-world forceful HRI applications.   
With respect to the peripersonal space comfort, while the participants showed a preference for the Comfort Planner configurations compared to the Random configurations, the difference was not as significant. During the experiments some participants expressed that they did not prefer to be very far away from the robot, possible suggesting that, while the peripersonal distance must be maximized up to a certain degree, there may be a distance after which it starts to negatively affect the collaboration. 

\begin{figure}[!t]
	\begin{center}
		\mbox{
			\subfigure[Random planner - Drilling]{{
					\label{fig:subfig:real:random-drill} 
					\includegraphics[width=1.6 in, angle=-0]{Experiment/fig/exp_RandomDrilling}}}
			\subfigure[Random planner - Cutting]{{
		\label{fig:subfig:real:random-cut}  
		\includegraphics[width=1.6 in, angle=-0]{Experiment/fig/exp_RandomCutting}}}	
		} 
		\mbox{
			\subfigure[Comfort based planner - Drilling]{{
					\label{fig:subfig:real:comfort-drill}  
					\includegraphics[width=1.6 in, angle=-0]{Experiment/fig/exp_OptimalDrilling}}}		
			
			\subfigure[Comfort based planner - Cutting]{{
					\label{fig:subfig:real:comfort-cut}  
					\includegraphics[width=1.6 in, angle=-0]{Experiment/fig/exp_OptimalCutting}}}					
		
		}		
		\caption{Cooperative drilling and cutting experiments.}
		\label{fig:realExperiments}
	\end{center}
\end{figure}



\begin{figure}[!t]
    \centering\includegraphics[width=0.9\columnwidth]{Experiment/fig/safetyAnalysis_wPoints}%
    \caption{Average peripersonal comfort perception from users (yellow dots) for drilling (left) and cutting (right) within the  \textbf{(a)} user defined object pose (black), \textbf{(b)} random planner (red), and \textbf{(c)} optimized pose (blue).}
\label{fig:baxter results:safety}
\end{figure}


\begin{figure}[!t]
    \centering\includegraphics[width=0.9\columnwidth]{Experiment/fig/comfortAnalysis_wPoints}%
    \caption{Average muscular comfort perception from users  (yellow dots) for drilling (left) and cutting (right) within the  \textbf{(a)} user defined object pose (black), \textbf{(b)} random planner (red), and \textbf{(c)} optimized pose (blue).}
\label{fig:baxter results:comfort}
\end{figure}




==> New folder/Introduction/Introduction.tex <==
\section{Introduction}
\label{sec:intro} 

In this paper, we are interested in the problem of a humanoid robot
manipulating an object in the close proximity of a human operator, who applies
a forceful operation such as drilling and cutting on the object. An instance is
shown in Fig.~\ref{fig:h-r drilling} where a human is drilling on a wooden
board firmly held by a humanoid robot at different configurations.
Theoretically, there may be infinite ways for the robot to grasp and position
the board and accordingly for the human to apply the desired force on it, among
which a large proportion of configurations are obviously uncomfortable for the human as shown
in Fig.~\ref{fig:subfig:uncomfort} and even unsafe as shown in Fig.~\ref{fig:subfig:unsafesafe}.
Human comfort and safety
during a forceful operation highly depends on how the human body is positioned and configured,
and therefore, where and how the robot positions its manipulators and the
object for the operation.  Under this circumstance, given a forceful operation to be applied by a
human operator, it is critical to empower the robot with the capability to plan
and position itself and the object at configurations which are not only stable,
but also comfortable for the human to perform the operation.  

In this context,
we propose a planner that enables a robot to grasp and position an object for a
forceful operation applied by a human that explicitly concerns human comfort
and force stability.  The final goal is to have an enhanced human-robot
interaction (HRI) experience with improved performance from both sides.

\begin{figure}[!t]
	\begin{center}
		\mbox{
			
			\subfigure[Too close to the robot]{{
					\label{fig:subfig:unsafesafe}  
					\includegraphics[width=1.6 in, angle=-0]{Introduction/figs/notSafe}}}
			
			\subfigure[High muscular effort]{{
					\label{fig:subfig:uncomfort}  
					\includegraphics[width=1.6  in, angle=-0]{Introduction/figs/notComfortable}}}			
		}
		\mbox{
	
			\subfigure[Unstable grasp]{{
					\label{fig:subfig:uncomfortSafe}  
					\includegraphics[width=1.6 in, angle=-0]{Introduction/figs/fail_drilling}}}
			
			\subfigure[Comfortable and stable]{{
					\label{fig:subfig:comfortsafe}  
					\includegraphics[width=1.6  in, angle=-0]{Introduction/figs/ComfortableSafe}}}			
		}
		\caption{Human-robot collaborative drilling on a board.}
		\label{fig:h-r drilling}
	\end{center}
\end{figure}

%\begin{figure}[thpb]
%	\begin{center}
%		\mbox{
%			
%			\subfigure[Object slides between grippers]{{
%					\label{fig:subfig:fail_cutting}  
%					\includegraphics[width=1.6 in, angle=-0]{Introduction/figs/fail_cutting}}}
%			
%			\subfigure[Object bends due to large torque]{{
%					\label{fig:subfig:fail_drilling}  
%					\includegraphics[width=1.6  in, angle=-0]{Introduction/figs/fail_drilling}}}			
%		}
%		\caption{Examples of unsafe grasps for cutting (a) and drilling (b).}
%		\label{fig:fail}
%	\end{center}
%\end{figure}


% There are three key problems our planner solves.


To quantify the human comfort during forceful interaction, we formulate a cost
based on human muscular features, kinematics and the involved forces.  First,
our planner produces %\textit{muscular-comfortable} 
solutions 
%for a human 
by minimizing a human \textit{muscular
comfort} cost, which quantifies the muscular
effort required for the human to perform a specific forceful operation on the
object.  
This metric, for example, predicts higher muscular comfort for the human 
in Fig.~\ref{fig:subfig:comfortsafe} and Fig.~\ref{fig:subfig:unsafesafe}, and lower muscular comfort for the human in Fig.~\ref{fig:subfig:uncomfort}, for the same task of drilling.
%The muscular comfort cost focuses on the physical sensation of the
%human body while applying a force at a certain configuration. It 
The muscular comfort metric predicts and
proactively instructs human to configurations which require less physical
joint-torque efforts to perform a forceful operation.
%, and, then plan the robot
%configuration, the robot grasp on the object, and the object position
%accordingly.


% Second, our planner minimizes the human's psychological weight by optimizing a cost of \textit{peripersonal-space} comfort.
% The peripersonal-space comfort concretizes a human's psychological sensations
% while working with a robot standing inside his peripersonal space. Minimizing
% the peripersonal-space comfort essentially positions the robot and the human
% at a distance far from each other, pulling the robot out of human's
% peripersonal space.
Nonetheless, through our initial experiments, we discovered that optimizing
only the muscular comfort is not sufficient. For example, while the human in Fig.~\ref{fig:subfig:unsafesafe} may have better muscular comfort compared to Fig.~\ref{fig:subfig:uncomfort}, he is dangerously close to the robot and is obstructed by the robot links.
Human behavior vary according to their assessment of the robot counterpart, and
human performance also depends on their level of trust and safety perception regarding the robot coworker \cite{2014_Lasota_Rossano_Shah__CASE,2015_Lasota_Shah__HF}. 
Furthermore, the human and robot may need to move before, during and after the forceful operation. Therefore, having enough space between them is important.
In this paper, to improve human awareness and safety perception, we exploit the concept of peripersonal space comfort. The idea is to allow humans to move and act within their peripersonal space% 
  \footnote{Peripersonal space is the space immediately surrounding our body, or the sector of space that closely surrounds a certain body part, in which multisensory and sensorimotor integration is enhanced \cite{2014_Bartolo_Carlier_Hassaini_Martin_Coello___FrontiersHN,1981_Rizzolatti_Scandolara_Matelli_Gentilucci___BehaviouralBrainResearch}. } 
  minimizing the perceived risk of robot intervention. Therefore, we propose a \textit{peripersonal-space cost} that is based on the distance between parts of the human and robot bodies.    
% 
%Take the examples in Fig.~\ref{fig:h-r drilling}, we can say the configuration in Fig.~\ref{fig:subfig:unsafesafe}  is more comfortable than the one in Fig.~\ref{fig:subfig:uncomfort}, in terms of muscular effort for the human to perform the drilling operation. However, the configuration in Fig.~\ref{fig:h-r drilling} positions the robot and object in a much closer distance from the human body, which would inevitably pose a bigger psychological pressure on the human and even endanger the human body. Apparently, the configuration in Fig.~\ref{fig:subfig:uncomfortSafe} is even worse. The robot in Fig.~\ref{fig:subfig:uncomfortSafe} positions itself and the object far away from the human. Even the human can take the initiative to step closer to the object, it is still too high for the human to reach.
%That is, none of the three configurations is comfortable or appropriate for the human to perform the drilling operation.
%Instead, in Fig.~\ref{fig:subfig:comfortsafe} the human is drilling at a relatively comfortable pose, with the distance to the robot being large enough to reduce spatial discomfort.
The configurations in Fig.~\ref{fig:subfig:comfortsafe} shows a configuration optimizing for both the muscular and the peripersonal-space comfort: the human is drilling at a relatively comfortable pose, with the distance to the robot being large enough to reduce spatial discomfort.


% Third, our planner guarantees force stability while planning for comfortable robot and object configurations for the human operator. 
Finally, ensuring robot capabilities to cope with the forceful task is also crucial, and cannot be decoupled from system analysis since different object/human poses results in different forces to cope. 
% 
Force stability checking involves choosing appropriate robot grasps on an
object and joint configurations to hold the object stable against the force
applied by the human. 
%It plays an important role in securing feasible and safe
%configurations for the forceful human-robot collaboration instance in our work.
A bad grasp of the object (as in Fig.~\ref{fig:subfig:uncomfortSafe}) may result in failed operations which would not only disturb the
fluency of HRI, but also pose serious danger to human
safety. For example, the object may slip through the fingers during a cutting
operation, or it may bend away
from the desired pose due to large torques around the gripper during a drilling
action as shown in Fig.~\ref{fig:subfig:uncomfortSafe}.
% 
This places an additional constraint: tightly coupled
human-robot kinematics and force stability must be guaranteed, while the human
comfort is optimized in the resulting space. 

In our previous work \cite{chen2018manipulation}, we have presented a manipulation planner for a robot to keep an object stable under changing external forces by
automatically deciding when and how to regrasp in a multi-step task scenario. 
Although improved robot performance has been achieved, human comfort during the interaction was ignored. To be more specific, the object pose was fixed in that work, which posed difficulties and discomfort for the human to perform the task. In real world applications, the resulting grasp/object pose may be crucial for the human experience, performance and safety. 
% . The planner particularly focuses on the scenario where a human may be applying forceful operations, e.g. cutting or drilling, on an object that the robot is holding. It produces an efficient plan by intelligently deciding when the robot should change its grasp on the object as the human applies the forces and also tries to choose subsequent grasps such that they will minimize the number of regrasps required in the long-term. However, in this work, the object pose is set to be fixed, which may pose difficulties and discomfort for the human to perform the task. 
Different from our previous work, the work in this paper focuses on planning
robot and object configurations that are not only stable but also comfortable
for the human to perform the forceful operation. It can be regarded as the
first step of planning fluid, comfortable and efficient human-robot
collaborative forceful manipulation. 
%Existing work in forceful human-robot collaboration mostly focuses on the control problem \cite{kosuge1997control,rozo2016learning,abi2017learning}, solving for the necessary stiffness of manipulator joints as as external force is applied, and assumes the object to be already grasped at pre-specified positions by the robot. Other similar work in planning for human-robot collaborations focuses on handing over an object to a human , or avoiding colliding a human working in the same workspace \cite{luo2017unsupervised,maeda2017probabilistic}.




==> New folder/Related/relatedwork.tex <==
\section{Related work}
\label{sec:related} 


Human-robot collaboration (HRC) has been interpreted from various aspects and tackled at different levels. 
Existing work in forceful HRC mostly addresses the control problem \cite{kosuge1997control,rozo2016learning}, solving for the necessary stiffness of manipulator joints as an external force is applied \cite{gopinathan2017user}, and assumes the object to be already grasped at pre-specified positions by the robot. 
Similar planning work mostly focuses on handover  \cite{sisbot2012human,strabala2013towards}, transportation \cite{rozo2016learning,solanes2018human}, or scenarios where the robot avoids colliding a human in the same workspace \cite{luo2018unsupervised,maeda2017probabilistic}. 
% 
Handover resembles our task in requiring the robot to position an object for a human. 
However, the physical interactions for handovers are usually 
not as intensive or physical demanding for both parts
thus planning has other priorities 
% momentary and light, thus planning preferred handover configurations can be simply divided into limited phases by first finding object transfer points 
\cite {sisbot2012human,parastegari2017modeling}. 
% 
Our task scenario differs in the existence of strong forceful interactions. % and their durative property, which put more requirements to the planner. 
Similar to handover, human-robot collaborative transportation connects a human and a robot together through a shared object 
but for a longer time. 
It requires the human and the robot to share load by holding an object at a desired orientation \cite{lawitzky2010load}, which is similar to finding appropriate grasps and robot configurations to keep an object stable in our work. 
% 
Human comfort and safety have been explicitly considered in human-aware motion planning for 
for object handover and transportation \cite{sisbot2012human,parastegari2017modeling,solanes2018human}. 
%  
With regard to forceful applications, Mansfeld et al. \cite{mansfeld2018safety} extend the safety analysis to general HRI and propose a new concept global safety assessment framework in practical HRC  applications, namely the safety map. 
% 
The excel works of Peternel et al. \cite {peternel2016adaptation,2017_Peternel_Kim_Ajoudani__Humanoids} should also be mentioned for addressing important topics in forceful HRC 
related to this work such as human ergonomics during forceful control co-operations and hand-over, where joint torques are taken into account through an offline identification technique but, still without proper knowledge on muscular activity---as well as safety perception and grasp stability.   
% 
Similar problem has also been addressed in \cite{2018_ICRA_Busch_Toussaint_Lopes} 
but considering an industrial ergonomic assessment based on payload mass and kinematics alone.  
% 
% 
% 
% \luisrm{
% In addition to comfort, Nico et al. work, }\cite{mansfeld2018safety}\luisrm{, should also be mentioned as it proposes a new concept global safety assessment framework in practical HRC  applications, namely the safety map.
% }
%
Indeed, despite the advances and contributions aforementioned, HRC still lacks  
efficient metrics for planning comfortable human-robot forceful collaborations 
explicitly considering muscular activation levels and human comfort perception, and planning object grasps and positioning. %olutions that cope with comfort whilst ensuring grasp stability. 
% in our work. 
% 
% 
% % 
% and human-aware motion  \cite {sisbot2012human,peternel2016adaptation,parastegari2017modeling}. However, there is still a lack of efficient metrics for planning comfortable human-robot forceful collaborations. % in our work. 



==> New folder/Safety/Safety.tex <==
\section{Peripersonal-space comfort}
\label{sec:Peripersonal} 

In this section, we define our metric quantifying the human's
peripersonal-space comfort for human-robot cooperative forceful manipulation.
We define this metric so that the optimization problem, presented in
Sec.~\ref{sec:defi}, can find solutions for which the human and robot body are
positioned at a comfortable distance from each other during collaboration.

%Similar to interactions among humans, in a human-robot collaboration, if robots stands too close to its human parnter, or even surround the human body, e.g., the robot hugs the human as shown in Fig.~\ref{fig:subfig:uncomfortSafe}, it will invade and occupy a large part of the human's peripersonal space, which, as a consequence, will cause a sense of discomfort, such as stress and anxiety, to the human.  Furthermore, the inappropriate spatial occupancy, in some cases may block the human's view, thus effecting the visibility of object held by the robot, such as the instance shown in Fig.~\ref{fig:subfig:unsafesafe}.  
%
%(Constraints brougnt about by Forceful operation). Unlike hand-overs in which the human and robot just reach and hold the object together momentarily, froceful operations usually requires strong and lasting interactions, thus placing more constraints on the configurations of the robot and object. For example, a too short distance will inevitably pose a potential danger to the human, especially when the human is involved in forceful operations.

In particular, for peripersonal comfort and safety, one would not want the human and
robot body to get too close to each other during cooperation. Therefore, we
define the peripersonal space comfort in terms of the distance
between the human and robot bodies. Given a human configuration,
$\textbf{\textit{q}}_{\text{h}}$, and pose, $_{\text{h}}{\textbf{\textit{T}}}$,
    we represent the set of points on the human body as
    $P_\text{h}(\textbf{\textit{q}}_{\text{h}},_{\text{h}}{\textbf{\textit{T}}})=\left\{p_\text{h}^1, p_\text{h}^2,...,p_\text{h}^n\right\}$
    where $p_\text{h}^i \in \mathbb{R}^3$.  Similarly, given a robot configuration
    $\textbf{\textit{q}}_{\text{r}}$, we represent the set of points on the
    robot body as $P_\text{r}(\textbf{\textit{q}}_{\text{r}})=\left\{p_\text{r}^1,
    p_\text{r}^2,...,p_\text{r}^m\right\}$  where $p_\text{r}^i \in \mathbb{R}^3$.
    (For clarity, in the rest of this work, we will simply use $P_\text{h}$ and $P_\text{r}$, dropping the arguments specifying the human/robot configurations and poses.)
Then, one can define the peripersonal comfort in terms of the distances
between these two set of points.

One option is to consider the minimum distance between the human and the robot,
and hypothesize the cooperation would be as comfortable as the minimum distance allows:
\begin{equation}\label{eq:peri_min_distance}
\text{Peripersonal}\left(\textbf{\textit{q}}_{\text{h}},\,\textbf{\textit{q}}_{\text{r}},\,_{\text{h}}{\textbf{\textit{T}}}\right)=
\min_{\forall p_\text{h} \in P_\text{h}, \forall p_\text{r} \in P_\text{r}} || p_\text{h} - p_\text{r} ||
\end{equation}
Then, the optimization process in Sec.~\ref{sec:defi} would be maximizing this minimum distance between the human and the robot.

While this metric may work well for different types of HRI,
it does not work well in the scenarios discussed in this work, since the
minimum distance between the human and the robot have a tight upper bound for
our tasks.  As shown in Fig.~\ref{fig:problem_define} the grippers of the robot
and the human hand on the tool are naturally the closest points. Thus,
maximizing the minimum distance will mostly only maximize the distance between
human hand and robot grippers, completely ignoring any other part of the body.

To address this issue and to take all points into account, one can instead consider the average distance over all points in the human body:
\begin{gather}\label{eq:dis_summin}
\text{Peripersonal}\left(\textbf{\textit{q}}_{\text{h}},\,\textbf{\textit{q}}_{\text{r}},\,_{\text{h}}{\textbf{\textit{T}}}\right)=
\frac{1}{|P_\text{h}|}\sum_{p_\text{h} \in P_\text{h}} \min_{\forall p_\text{r} \in P_\text{r}} || p_\text{h} - p_\text{r} ||
\end{gather}
While this metric takes all human body points into account, it also has a
problem: the large distances dominate this metric.  If a human configuration
has one point that is very far away from the robot but many other points that
are very close to the robot, then, 
this metric may provide misleading results.
%using the metric in
%Eq.~\ref{eq:dis_summin}, this configuration may have a better peripersonal
%comfort metric than a configuration where most human body points are at a safe
%but medium distance from the robot.

This suggests we need a metric that takes all human body points into account,
but that also gives more weight to points with small distances to the robot and less
weight to points with large distances to the robot. Therefore, we propose the peripersonal space metric:
\begin{gather}\label{eq:dis_weighted}
\text{Peripersonal}\left(\textbf{\textit{q}}_{\text{h}},\,\textbf{\textit{q}}_{\text{r}},\,_{\text{h}}{\textbf{\textit{T}}}\right)=
\frac{1}{|P_\text{h}|}\sum_{p_\text{h} \in P_\text{h}} w(p_\text{h}) \min_{\forall p_\text{r} \in P_\text{r}} || p_\text{h} - p_\text{r} ||
\end{gather}
where $w(p_\text{h})$ is the weight of the point $p_\text{h}$ defined as
\begin{equation}\label{weight}
    w(p_\text{h})
    =1-\frac{\min_{\forall p_\text{r} \in P_\text{r}} || p_\text{h} - p_\text{r} ||}{\sum_{p_\text{h} \in P_\text{h}} \min_{\forall p_\text{r} \in P_\text{r}} || p_\text{h} - p_\text{r} ||}
\end{equation}
It associates a small distance with a large weight, thus controlling all distances efficiently.
Eq.~\ref{eq:dis_weighted}~and~\ref{weight} together define the peripersonal comfort metric used in this work. 

%By optimizing it, our planner positions the robot as sufficiently far as possible from the human's personal space, but guaranteeing the object is reachable for the human.



%%%%%%%%%%%%%%%%%%%%%5

%For a given force operation $(^\text{o}\textbf{\textit{f}},\, _{\text{t}}^{\text{o}}{\textbf{\textit{T}}})$, human and robot configuration $\left(\textbf{\textit{q}}_{\text{h}},\,\textbf{\textit{q}}_{\text{r}},\,_{\text{h}}{\textbf{\textit{T}}}\right)$, 
%we define the human's peripersonal comfort $\text{Peripersonal}\left(\textbf{\textit{q}}_{\text{h}},\,\textbf{\textit{q}}_{\text{r}},\,_{\text{h}}{\textbf{\textit{T}}}\right)$ over the distance between the human  and the robot:
%\begin{equation}\label{equ:peri_distance}
%\text{Peripersonal}\left(\textbf{\textit{q}}_{\text{h}},\,\textbf{\textit{q}}_{\text{r}},\,_{\text{h}}{\textbf{\textit{T}}}\right)=\text{Distance}\left(\textbf{\textit{q}}_{\text{h}},\,\textbf{\textit{q}}_{\text{r}},\,_{\text{h}}{\textbf{\textit{T}}}\right)
%\end{equation}
%This requires the planner to decide on appropriate schemes for distance computing, which highly depends on the human and robot models.  
%\begin{figure}[thpb]
%	\begin{center}
%		\mbox{
%			
%			\subfigure[human skeleton-model]{{
%					\label{fig:subfig:humanmodel}  
%					\includegraphics[width=1.6 in, angle=-0]{Safety/humanskeleton}}}
%			
%			\subfigure[robot skeleton-model]{{
%					\label{fig:subfig:robotmodel}  
%					\includegraphics[width=1.6  in, angle=-0]{Safety/humanskeleton}}}			
%		}
%		\caption{Human and robot skeleton model (polish later).}
%		\label{fig:model}
%	\end{center}
%\end{figure}
%
%In this work, we  model the human's  geometry using a set of skeleton points $P_\text{h}=\left\{p_\text{h}^1, p_\text{h}^2,...,p_\text{h}^n\right\}$  without radius, which are  attached  and well distributed on the human body, such as joints, limb centers and human head. 
%Especially, as shown in Fig.~\ref{fig:model}, we put more points on human arms, which are more vulnerable when the human performs a forceful operation with the assistance of the robot. These points together depicts the skeleton structure of human body. Similarly, we represent the robot with a limited set of points $P_\text{r}=\left\{p_\text{r}^1, p_\text{r}^2,...,p_\text{r}^m\right\}$ in this work. 
%
%In this context, For given human and robot configuration $\left(\textbf{\textit{q}}_{\text{h}},\,\textbf{\textit{q}}_{\text{r}},\,_{\text{h}}{\textbf{\textit{T}}}\right)$, one option to measure their distance is to compute the shortest distance between the human and the robot:
%\begin{equation}\label{min-dis}
%\text{Distance}\left(\textbf{\textit{q}}_{\text{h}},\,\textbf{\textit{q}}_{\text{r}},\,_{\text{h}}{\textbf{\textit{T}}}\right)=\text{distance\_min}\left (P_\text{h},P_\text{r}\right )
%\end{equation}
%
%Equation~\ref{min-dis} computes all distances between points from the set $P_\text{h}$ and $P_\text{r}$ and then returns the shortest one. It
%works well for scenarios in which the interactions between the human and the robot are monetary and light, such as handover \cite{sisbot2012human}. 
%However, in the scenarios discussed in this work, when the human performs the operation, as shown in Fig.~\ref{fig:problem_define} the two grippers are naturally closest to the human body/hand compared with other parts of robot body. Thus, maximizing the minimum distance will mostly only maximize the distance between human hand and robot grippers.
%
%Another option for the planer is to sum up all minimum distances of points in $P_\text{h}$ to the robot $P_\text{r}$, and maximize the sum, that is:
%\begin{gather}\label{dis_summin}
%\text{Distance}\left(\textbf{\textit{q}}_{\text{h}},\,\textbf{\textit{q}}_{\text{r}},\,_{\text{h}}{\textbf{\textit{T}}}\right)=\sum_{i=1}^{n}\text{distance\_min}\left (p_\text{h}^i,P_\text{r}\right ) 
%\end{gather}
%
%Equation~\ref{dis_summin} can efficiently control the entire distance between the robot and human body. However, this formulation treats all distances at different order of magnitudes equally. Consequently, the effect of some small distances, such as the distances between the human hand and robot grippers, will be weakened when directly summoned up as Equation~\ref{dis_summin}, thus these distances will not be well optimized.
%
%To solve this problem, we introduce a self-adaptive strategy by computing the distance as the weighted-sum of the minimum distances:
%\begin{gather}\label{dis_weighted}
%\text{Distance}\left(\textbf{\textit{q}}_{\text{h}},\,\textbf{\textit{q}}_{\text{r}},\,_{\text{h}}{\textbf{\textit{T}}}\right)=\sum_{i=1}^{n}w_{i}\times \text{distance\_min}\left (p_\text{h}^i,P_\text{r}\right ) 
%\end{gather}
%where $w_i$ is the weight defined as
%\begin{equation}\label{weight}
%	w_{i}
%=1-\frac{\text{distance\_min}\left (p_\text{h}^i,P_\text{r}\right)}{\sum_{j=1}^{n}\text{distance\_min}\left (p_\text{h}^j,P_\text{r}\right)}
%\end{equation}
%It associates a small distance with a large weight, thus controlling all distances efficiently.
%Equation~\ref{equ:peri_distance},~\ref{dis_weighted},~\ref{weight} together define the peripersonal comport metric used in this work. 
%By optimizing it, the planner positions the robot as sufficiently far as possible from the human's personal space, but guaranteeing the object is reachable for the human.






==> New folder/Stability/Stability.tex <==
\section{Stability Checking}
\label{sec:Feasibility} 

In addition to optimizing the muscular and peripersonal space comfort, the
optimization problem presented in Eq.~\ref{optimization} also makes sure that
the robot configuration, $\textbf{\textit{q}}_{\text{r}}$, the object pose,
$_{\text{o}}\textbf{\textit{T}}$, and the grasp, $\textit{\textbf{g}}$, are
chosen such that the object and the robot are stable during the application of the
force on the object by the human. This constraint is represented by the
Is\_stable function in Eq.~\ref{optimization}.  This function validates that:
\begin{itemize}
    \item The torque distribution on the robot arms' joints will not exceed the torque limits; 
    \item The grip forces, e.g. the frictional forces between robot fingers, will be able to resist the external force applied on the object.
\end{itemize}

Due to space limitation we skip the mathematical formulation
here, which can be found in our previous work
\cite{chen2018manipulation}, in
Section III-A-1, titled \textit{Stability Check}.  





==> New folder/problemdefinition/problemdefinition.tex <==
\section{Problem formulation}
\label{sec:defi} 

We are interested in the problem of finding optimal robot and object configurations for forceful human-robot collaborative manipulation, in which a human performs a specific forceful operation such as drilling and cutting, on an object stably held by a robot in the shared environment.

\begin{figure}[!t]
	\begin{center}
		\mbox{
			\subfigure{{
					\label{fig:subfig:problem_define}  
					\includegraphics[width=3.0 in,height=2.5 in, angle=-0]{problemdefinition/problemdefine}}}			
		}
		
		\caption{human-tool-object-robot configuration.}
		\label{fig:problem_define}
	\end{center}
\end{figure}



As shown in Fig.~\ref{fig:problem_define}, when the human applies the force, the human and robot geometry and kinematics are tightly coupled by means of the tool-object system. We assume a  fixed grasp  for the human to grasp a specific tool, and therefore a fixed kinematic transformation between the human hand and the tool. 
We assume a tool frame ${\sum}_{\text{t}}$ attached at the tooltip and a human frame attached at the shoulder ${\sum}_{\text{h}}$. Since the operational force is applied exactly at the contact points between the object and the tooltip, the force position (e.g., the point to drill on the object) can be specified by the pose  of the tooltip $_{\text{t}}^{\text{o}}\textbf{\textit{T}}$ in the object\footnote{We use superscripts at the top-left of the variables to distinguish the coordinate frames with respect to which the variables are expressed.} frame ${\sum}_{\text{o}}$. 

In this context, a forceful operation can be specified by a tuple: \begin{equation}\label{key}
(^\text{o}\textbf{\textit{f}},\, _{\text{t}}^{\text{o}}{\textbf{\textit{T}}})
\end{equation}
where $^\text{o}\textbf{\textit{f}}$ is the 6D generalized force vector.
We assume that such an operation is provided to our system; i.e. the pose of the force application (e.g. the drill point on the board) and the expected force (e.g. the expected drilling force).
%For clarity of explanation and because 

Besides, we use a humanoid robot in our experiments, thus assuming the robot has two dexterous manipulators and each manipulator is equipped with a parallel gripper. However, our formulation can be easily extended to systems with more manipulators. Given a forceful operation $(^\text{o}\textbf{\textit{f}},\, _{\text{t}}^{\text{o}}{\textbf{\textit{T}}})$, the composite configuration for the human robot collaboration can be fully specified by five variables\footnote{Without loss of generality, we assume the robot frame ${\sum}_{\text{r}}$ coincides with the world frame, thus ommitting superscripts for variables if they are defined in the world/robot frame.} ${\textbf{\textit{q}}=\left(\textbf{\textit{q}}_{\text{h}},\,\textbf{\textit{q}}_{\text{r}},\,_{\text{h}}\textbf{\textit{T}},\,_{\text{o}}\textbf{\textit{T}},\textit{\textbf{g}}\right)}$, where:
\begin{itemize}
    \item $\textbf{\textit{q}}_{\text{h}}$ refers to human body configuration\footnote{In this work, the muscular comfort metric (see Sec.~\ref{sec:Muscular}) only takes human arm configuration into account, and therefore within this paper we use $q_{\text{h}}$ to refer to human arm configuration.  However, the optimization problem we define in this section is general to whole body configurations.};
	\item $\textbf{\textit{q}}_{\text{r}}=\left\{\textbf{\textit{q}}_{\text{rl}},\,\textbf{\textit{q}}_{\text{rr}}\right\}$ refers to the robot configuration, where $\textbf{\textit{q}}_{\text{rl}}$ and $\textbf{\textit{q}}_{\text{rr}}$ denote the left and right arm configuration respectively;
	\item $_{\text{h}}^{\text{}}\textbf{\textit{T}}$ describes the 6D pose of the human body in the robot frame;
	\item  $_{\text{o}}\textbf{\textit{T}}$ refers to the 6D object pose in the robot frame;
	\item $\textit{\textbf{g}}$ denotes a grasp using the pose of gripper(s)  with respect to the object. To be more specific, in this paper, $\textit{\textbf{g}}$ refers to a bimanual grasp specifying the pose of both left and right grippers on the object. 	
\end{itemize}
Note that there is redundancy in this definition. Specifically, given a robot configuration $\textbf{\textit{q}}_{\text{r}}$ and object pose $_{\text{o}}\textbf{\textit{T}}$, the corresponding grasp comfiguration $\textit{\textbf{g}}$ can be computed via robot forward kinematics.

\subsection{Optimization}

For a given force operation $(^\text{o}\textbf{\textit{f}},\, _{\text{t}}^{\text{o}}{\textbf{\textit{T}}})$, our planner aims at finding the robot configuration $\textbf{\textit{q}}_{\text{r}}$ and object pose  $_{\text{o}}\textbf{\textit{T}}$, such that the object is stably grasped against the applied force \textit{and} the human comfort is maximized:
\begin{equation}\label{optimization}
\begin{split}
&\textbf{\textit{q}}_{\text{r}}^*,\,_{\text{o}}\textbf{\textit{T}}^*=
\mathop{\arg\max}_{\textbf{\textit{q}}_{\text{r}},\,_{\text{o}}\textbf{\textit{T}}}\,\text{Comfort}\left(\textbf{\textit{q}}_{\text{r}},\,_{\text{o}}\textbf{\textit{T}},\,^\text{o}\textbf{\textit{f}},\, _{\text{t}}^{\text{o}}{\textbf{\textit{T}}}\right)\\
&\text{s.t.\,}\,\,\text{Is\_stable}\left(\textbf{\textit{q}}_{\text{r}},\,\textit{\textbf{g}},\,^\text{o}\textbf{\textit{f}},\, _{\text{t}}^{\text{o}}{\textbf{\textit{T}}}\right)
\end{split}
\end{equation}

Function $\text{Is\_stable}$ checks whether the robot at the configuration $\textbf{\textit{q}}_{\text{r}}$ is able to resist the operation force $^\text{o}\textbf{\textit{f}}$ with the grasp $\textit{\textbf{g}}$ on the object via static equilibrium, which will be discussed with more detail in Sec.~\ref{sec:Feasibility}. 

The optimization problem requires us to compute the value of $\text{Comfort}$,
which we use to represent the total human comfort. We propose to
model this value using two components: human's \textit{muscular} comfort and
human's \textit{peripersonal-space} comfort.
Here we assume the existence of functions which quantify these comfort metrics: 
\begin{itemize}
    \item $\text{Muscular}\left(\textbf{\textit{q}}_{\text{h}}, \, _{\text{h}}{\textbf{\textit{T}}},  \, ^{\text{o}}{\textbf{\textit{f}}}, \, _{\text{t}}^{\text{o}}{\textbf{\textit{T}}}, \, _{\text{o}}{\textbf{\textit{T}}} \right)$: This function
    returns a scalar value quantifying the muscular comfort of the human given
    the human configuration, pose, and the forceful operation to be applied. We
    present how we model this function in Sec.~\ref{sec:Muscular}.  
    \item $\text{Peripersonal}\left(\textbf{\textit{q}}_{\text{h}},\,_{\text{h}}{\textbf{\textit{T}}},\,\textbf{\textit{q}}_{\text{r}}\right)$:
        This function returns a scalar value quantifying the peripersonal-space
        comfort of the human given the human configuration, pose, and the robot
        configuration.  We present how we model this function in Sec.~\ref{sec:Peripersonal}.  
\end{itemize}

%The two comfort metrics are functions of human configuration $\textbf{\textit{q}}_{\text{h}}$, human pose $_{\text{h}}{\textbf{\textit{T}}}$, robot configuration $^{\text{o}}{\textbf{\textit{f}}}$ and operation force $^{\text{o}}{\textbf{\textit{f}}}$. They are used together as costs to determine the optimal robot configuration $\textbf{\textit{q}}_{\text{r}}$ and object $\textbf{\textit{q}}_{\text{o}}$. 
For a given forceful operation, our goal is to determine a robot configuration $\textbf{\textit{q}}_{\text{r}}$ and object pose $_{\text{o}}\textbf{\textit{T}}$ that maximizes these two costs.
However, computing these comfort metrics requires us to know the human configuration $\textbf{\textit{q}}_{\text{h}}$.
But, for a given robot configuration $\textbf{\textit{q}}_{\text{r}}$ and object pose  $_{\text{o}}\textbf{\textit{T}}$, 
the human can choose many different body configurations and poses to perform an operation. This raises the question of how the human will choose her configuation and pose, based on which we can compute the $\text{Comfort}$ value in Eq.~\ref{optimization}.

Given the robot configuration $\textbf{\textit{q}}_{\text{r}}$, object pose  $_{\text{o}}\textbf{\textit{T}}$ and the operation $(^\text{o}\textbf{\textit{f}},\, _{\text{t}}^{\text{o}}{\textbf{\textit{T}}})$, 
we define the set of all \textit{feasible} human pose and configuration combinations as
$Q_h\left(\textbf{\textit{q}}_{\text{r}},\,_{\text{o}}\textbf{\textit{T}},\,^\text{o}\textbf{\textit{f}},\, _{\text{t}}^{\text{o}}{\textbf{\textit{T}}}\right)$. 
By feasible, here we mean human poses and configurations that satisfy the stability constraints and 
the kinematic constraints (i.e., that puts the tool frame ${\sum}_{\text{t}}$ at the forceful operation point on the object as shown in Fig.~\ref{fig:problem_define}).
In other words, $Q_h$ includes the human poses and configurations the human can choose from to successfully perform the task.
Then, one can model the $\text{Comfort}$ using different schemes: 
\begin{itemize}
    \item One option is to take the average comfort value of all feasible human configurations and poses. Assuming $Q_h$ is a discretised set:
\begin{equation}\label{average_comfort}
\begin{split}
		\text{Comfort}\left(\textbf{\textit{q}}_{\text{r}},\,_{\text{o}}\textbf{\textit{T}},\,^\text{o}\textbf{\textit{f}},\, _{\text{t}}^{\text{o}}{\textbf{\textit{T}}}\right)=\\
        \underset{\textbf{\textit{q}}_{\text{h}},\,_{\text{h}}{\textbf{\textit{T}}} \in  Q_h}{\sum{\{w_{\text{M}}}}{\text{Muscular}\left(\textbf{\textit{q}}_{\text{h}}, _{\text{h}}{\textbf{\textit{T}}},  \, ^{\text{o}}{\textbf{\textit{f}}}, \, _{\text{t}}^{\text{o}}{\textbf{\textit{T}}} \right) }\\
{+w_{\text{P}}\text{Peripersonal}\left(\textbf{\textit{q}}_{\text{h}},\,\textbf{\textit{q}}_{\text{r}},\,_{\text{h}}{\textbf{\textit{T}}}\right)}\}/ | Q_h |
\end{split}
\end{equation}
Where $w_{\text{M}}$ and $w_{\text{P}}$ are weights. 
$| Q_h |$ indicates the size of $Q_h$. Note that the arguments to $Q_h$ is dropped above for clarity, but it is important to note that the set $Q_h$ is determined by the same arguments to Comfort function.

\item Another option is to assume the human will choose the most comfortable body configuration from among the feasible set: 
    %$\textbf{\textit{q}}_{\text{h}}$ and pose $_{\text{h}}{\textbf{\textit{T}}}$. Then for a given force operation $(^\text{o}\textbf{\textit{f}},\, _{\text{t}}^{\text{o}}{\textbf{\textit{T}}})$, the $\text{Comfort}$ is defined as
\begin{equation}\label{most}
\begin{split}
\text{Comfort}\left(\textbf{\textit{q}}_{\text{r}},\,_{\text{o}}\textbf{\textit{T}},\,^\text{o}\textbf{\textit{f}},\, _{\text{t}}^{\text{o}}{\textbf{\textit{T}}}\right)=\\
\underset{\textbf{\textit{q}}_{\text{h}},\,_{\text{h}}{\textbf{\textit{T}}} \in  Q_h }{\max\{w_{\text{M}}}{\text{Muscular}\left(\textbf{\textit{q}}_{\text{h}}, _{\text{h}}{\textbf{\textit{T}}},  \, ^{\text{o}}{\textbf{\textit{f}}}, \, _{\text{t}}^{\text{o}}{\textbf{\textit{T}}} \right) }\\
{+w_{\text{P}}\text{Peripersonal}\left(\textbf{\textit{q}}_{\text{h}},\,\textbf{\textit{q}}_{\text{r}},\,_{\text{h}}{\textbf{\textit{T}}}\right)}\}
\end{split}
\end{equation}

\end{itemize}

In the rest of this work we assume the human is optimal and therefore adopts the latter option, and we solve the optimization problem defined by Eq.~\ref{optimization} and~\ref{most}. The problem can alternatively also be solved for Eq.~\ref{optimization} and~\ref{average_comfort}.



